Numerical analysis of non-local calculus on finite weighted graphs, with application to reduced-order modelling of dynamical systems

We present an approach to reduced-order modelling that builds off recent graph-theoretic work for representation, exploration, and analysis of computed states of physical systems (Banerjee et al., Comp. Meth. App. Mech. Eng., 351, 501-530, 2019). We extend a non-local calculus on finite weighted graphs to build such models by exploiting polynomial expansions and Taylor series. In the general framework for non-local calculus on graphs, the graph edge weights are intricately linked to the embedding of the graph, and consequently to the definition of the derivatives. In a previous communication (Duschenes and Garikipati, arXiv:2105.01740), we have shown that radially symmetric, continuous edge weights derived from, for example Gaussian functions, yield inconsistent results in the resulting non-local derivatives when compared against the corresponding local, differential derivative definitions. Taking inspiration from finite difference methods, we algorithmically compute edge weights, considering the embedding of the local neighborhood of each graph vertex. Given this procedure, we ensure the consistency of the non-local derivatives in this setting, a crucial requirement for numerical applications. We show that we can achieve any desired orders of accuracy of derivatives, in a chosen number of dimensions without symmetry assumptions in the underlying data. Finally, we present two example applications of extracting reduced-order models using this non-local calculus, in the form of ordinary differential equations from parabolic partial differential equations of progressively greater complexity.

==> figures/model_diffusion_local_.tex <==
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} + {\gamma}^{{{{{F}_{-}}}^{}}}{{{{F}_{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} + {\gamma}^{{{{{F}_{-}}}^{}}}{{{{F}_{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} + {\gamma}^{{{{{F}_{-}}}^{}}}{{{{F}_{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} + {\gamma}^{{{{{F}_{-}}}^{}}}{{{{F}_{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + {\gamma}^{{{\varphi_{5{}}}^{}}}{{\varphi_{5{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}} + {\gamma}^{{{{\varphi}_{5{-}}}^{}}}{{{\varphi}_{5{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{{{F}^{\prime}_{-}}}^{}}}{{{{F}^{\prime}_{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + {\gamma}^{{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}} + {\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = {\gamma}^{{{\varphi_{{}}}^{}}}{{\varphi_{{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 5.309\cdot 10^{-2}{{\varphi_{{}}}^{}} - 2.497\cdot 10^{-2}{{\varphi_{3{}}}^{}} - 1.140\cdot 10^{-3}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.002\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 2.834\cdot 10^{-3}{{{{F}^{\prime}_{-}}}^{}} + 3.545\cdot 10^{-3}{{{\varphi}_{5{-}}}^{}} + 6.796\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + 1.533\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 3.924\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} + 1.128\cdot 10^{-4}{{\varphi_{5{}}}^{}} - 3.285\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} - 3.162\cdot 10^{-4}{{{{F}_{-}}}^{}} - 4.219\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}} - 2.539\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}} - 1.665\cdot 10^{-4}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.844\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.397\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 3.494\cdot 10^{-4}{{{{F}^{\prime}_{-}}}^{}} + 1.649\cdot 10^{-4}{{{\varphi}_{5{-}}}^{}} + 1.371\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 3.557\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 7.127\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} - 1.968\cdot 10^{-4}{{\varphi_{5{}}}^{}} + 1.635\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} + 1.160\cdot 10^{-5}{{{{F}_{-}}}^{}} - 8.097\cdot 10^{-6}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}} - 5.122\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.827\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.374\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 1.497\cdot 10^{-4}{{{{F}^{\prime}_{-}}}^{}} + 2.243\cdot 10^{-4}{{{\varphi}_{5{-}}}^{}} + 1.357\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 2.631\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 5.102\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} - 3.387\cdot 10^{-4}{{\varphi_{5{}}}^{}} - 2.219\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} - 3.326\cdot 10^{-5}{{{{F}_{-}}}^{}} - 7.189\cdot 10^{-7}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla_2 c_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.827\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.374\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 1.497\cdot 10^{-4}{{{{F}^{\prime}_{-}}}^{}} + 2.238\cdot 10^{-4}{{{\varphi}_{5{-}}}^{}} + 1.356\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 2.627\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 5.071\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} - 3.373\cdot 10^{-4}{{\varphi_{5{}}}^{}} - 2.216\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}} - 3.289\cdot 10^{-5}{{{{F}_{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.824\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.387\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 1.505\cdot 10^{-4}{{{{F}^{\prime}_{-}}}^{}} + 2.370\cdot 10^{-4}{{{\varphi}_{5{-}}}^{}} + 1.372\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 2.414\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 4.106\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} - 3.688\cdot 10^{-4}{{\varphi_{5{}}}^{}} - 1.919\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{3{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.861\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.382\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} - 5.786\cdot 10^{-5}{{{{F}^{\prime}_{-}}}^{}} + 1.503\cdot 10^{-4}{{{\varphi}_{5{-}}}^{}} + 1.368\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 1.575\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 2.457\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}} - 3.464\cdot 10^{-4}{{\varphi_{5{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.901\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.009\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 7.303\cdot 10^{-5}{{{{F}^{\prime}_{-}}}^{}} + 4.287\cdot 10^{-5}{{{\varphi}_{5{-}}}^{}} + 9.912\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 1.279\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}} - 7.248\cdot 10^{-5}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{F_{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.899\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.002\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 9.767\cdot 10^{-5}{{{{F}^{\prime}_{-}}}^{}} + 4.833\cdot 10^{-5}{{{\varphi}_{5{-}}}^{}} + 9.853\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}} - 1.098\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{4{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.897\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.007\cdot 10^{-3}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 7.288\cdot 10^{-5}{{{{F}^{\prime}_{-}}}^{}} + 4.939\cdot 10^{-5}{{{\varphi}_{5{-}}}^{}} + 9.962\cdot 10^{-4}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.893\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.062\cdot 10^{-5}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 5.844\cdot 10^{-5}{{{{F}^{\prime}_{-}}}^{}} + 5.886\cdot 10^{-5}{{{\varphi}_{5{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.914\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.429\cdot 10^{-5}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.117\cdot 10^{-4}{{{{F}^{\prime}_{-}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.914\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}} + 1.121\cdot 10^{-5}{{\frac{{\delta}^{} \Psi}{{\delta} {\varphi_{{}}}^{}}}^{}{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.000{{\varphi_{{}}}^{}} - 1.000{{\varphi_{3{}}}^{}} - 9.932\cdot 10^{-4}{{{\varphi}_{\scriptscriptstyle{\nabla^2_{-}}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 1.001{{\varphi_{{}}}^{}} - 1.037{{\varphi_{3{}}}^{}}$
$\frac{{\delta}^{} \varphi_{{}}}{{\delta} {t}^{}} = 0.162{{\varphi_{{}}}^{}}$


==> figures/model_diffusion_nonlocal.tex <==
\begin{subequations}
\renewcommand{\theequation}{\arabic{parentequation}~-~\the\numexpr6+7-1-\value{equation}\relax}
\begin{equation}
\begin{aligned}
{M_{\varphi}} =&~	 {\gamma}^{{{M}^{}{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}} + {\gamma}^{{{M}^{}{\varphi_{1{}}}^{}}}{{\varphi_{1{}}}^{}} + {\gamma}^{{{M}^{}{\bar{\varphi}_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\bar{\varphi}_{\scriptscriptstyle{\nabla^2_{}}}}^{}} + {\gamma}^{{{M}^{}{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}
\\
{\mathcal{E}_{\varphi}} =&~ {\gamma}^{{{{F^{\prime}_{}}}^{}}}{{{F^{\prime}_{}}}^{}}~+~{\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}~+~{\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{\varphi_{4{}}}^{}}}{{\varphi_{4{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{5{}}}^{}}}{{\bar{\varphi}_{5{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{2{}}}^{}}}{{\bar{\varphi}_{2{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{4{}}}^{}}}{{\bar{\varphi}_{4{}}}^{}}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
{M_{\varphi}} =&~ {\gamma}^{{{M}^{}{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{M}^{}{\varphi_{1{}}}^{}}}{{\varphi_{1{}}}^{}}~+~{\gamma}^{{{M}^{}{\bar{\varphi}_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\bar{\varphi}_{\scriptscriptstyle{\nabla^2_{}}}}^{}}
\\
{\mathcal{E}_{\varphi}} =&~ {\gamma}^{{{{F^{\prime}_{}}}^{}}}{{{F^{\prime}_{}}}^{}}~+~{\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}~+~{\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{\varphi_{4{}}}^{}}}{{\varphi_{4{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{5{}}}^{}}}{{\bar{\varphi}_{5{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{2{}}}^{}}}{{\bar{\varphi}_{2{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{4{}}}^{}}}{{\bar{\varphi}_{4{}}}^{}}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
{M_{\varphi}} =&~ {\gamma}^{{{M}^{}{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{M}^{}{\varphi_{1{}}}^{}}}{{\varphi_{1{}}}^{}}
\\
{\mathcal{E}_{\varphi}} =&~ {\gamma}^{{{{F^{\prime}_{}}}^{}}}{{{F^{\prime}_{}}}^{}}~+~{\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}~+~{\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{\varphi_{4{}}}^{}}}{{\varphi_{4{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{5{}}}^{}}}{{\bar{\varphi}_{5{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{2{}}}^{}}}{{\bar{\varphi}_{2{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{4{}}}^{}}}{{\bar{\varphi}_{4{}}}^{}}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
{M_{\varphi}} =&~ {\gamma}^{{{M}^{}{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}
\\
{\mathcal{E}_{\varphi}} =&~ {\gamma}^{{{{F^{\prime}_{}}}^{}}}{{{F^{\prime}_{}}}^{}}~+~{\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}~+~{\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{\varphi_{4{}}}^{}}}{{\varphi_{4{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{5{}}}^{}}}{{\bar{\varphi}_{5{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{2{}}}^{}}}{{\bar{\varphi}_{2{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{4{}}}^{}}}{{\bar{\varphi}_{4{}}}^{}}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
{M_{\varphi}} =&~ 0
\\
{\mathcal{E}_{\varphi}} =&~ {\gamma}^{{{{F^{\prime}_{}}}^{}}}{{{F^{\prime}_{}}}^{}}~+~{\gamma}^{{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}}{{\varphi_{\scriptscriptstyle{\nabla^2_{}}}}^{}}~+~{\gamma}^{{{\varphi_{3{}}}^{}}}{{\varphi_{3{}}}^{}}~+~{\gamma}^{{{\varphi_{4{}}}^{}}}{{\varphi_{4{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{5{}}}^{}}}{{\bar{\varphi}_{5{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{2{}}}^{}}}{{\bar{\varphi}_{2{}}}^{}}~+~{\gamma}^{{{\bar{\varphi}_{4{}}}^{}}}{{\bar{\varphi}_{4{}}}^{}}
\end{aligned}
\end{equation}
\end{subequations}

==> figures/model_psi_OLS_Ridge17_nonlocal.tex <==
\begin{align}
{\Psi}_{\textrm{OLS - Continuous}} =&~ {{\Psi}_{}}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}{\Delta {\bar{\varphi}}_{}}^{2} \label{eq:psi_model_OLS}\\
+&~ {\gamma}^{{\bar{E}}_{12}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{12} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{12}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{E}}_{12}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{12} \delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{12}}^{} {\Delta {\bar{\varphi}}_{}}^{2} \nonumber \\
+&~ {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{22}{\bar{E}}_{11}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{E}}_{11}}^{} \nonumber \\
+&~ {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{2} + {\gamma}^{{\bar{E}}_{22}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{} \nonumber \\
+&~ {\gamma}^{{\bar{E}}_{11}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{E}}_{22}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}, \nonumber \\ \nonumber \\
{\Psi}_{\textrm{Ridge - Continuous}} =&~ {{\Psi}_{}}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}{\Delta {\bar{\varphi}}_{}}^{2} \label{eq:psi_model_Ridge17} \\
+&~ {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{4}}{\Delta {\bar{\varphi}}_{}}^{4} + {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{22}{\bar{E}}_{11}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{E}}_{11}}^{} \nonumber \\
+&~ {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{11}{\bar{E}}_{11}{\bar{E}}_{11}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{11} \delta {\bar{E}}_{11} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3} + {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} \nonumber \\
+&~ {\gamma}^{{\bar{E}}_{12}}\frac{{\delta}^{} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{12}}^{}}{\Delta {\bar{E}}_{12}}^{} + {\gamma}^{{\bar{E}}_{11}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{\varphi}}_{}}^{} \nonumber \\
+&~ {\gamma}^{{\bar{E}}_{22}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{E}}_{22}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}. \nonumber 
\end{align}


==> figures/model_psi_OLS_local.tex <==
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.604\cdot 10^{-3}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 1.050\cdot 10^{-3}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 6.419\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 1.350\cdot 10^{-4}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 8.414\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 1.786\cdot 10^{-16}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 6.209\cdot 10^{-3}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.951\cdot 10^{-2}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}} + 5.335\cdot 10^{-8}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.531\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 1.796\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 1.511\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 5.060\cdot 10^{-8}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 2.442\cdot 10^{-12}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 4.944\cdot 10^{-20}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.468\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}} + 3.155\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.578\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 1.750\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 2.234\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 4.539\cdot 10^{-8}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 2.181\cdot 10^{-12}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 4.431\cdot 10^{-20}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 2.236\cdot 10^{-6}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.481\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 2.003\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 2.646\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 3.074\cdot 10^{-8}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.448\cdot 10^{-12}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 2.786\cdot 10^{-20}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.492\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 2.214\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 2.977\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 8.835\cdot 10^{-9}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 2.280\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.436\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 2.224\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 2.672\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}} + 8.940\cdot 10^{-10}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.509\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 2.366\cdot 10^{-5}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}} + 3.083\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{12}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.546\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 2.084\cdot 10^{-6}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.537\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})$


==> figures/model_psi_Ridge17_local.tex <==
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + {{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + {{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) + {{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.054\cdot 10^{-3}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.379\cdot 10^{-8}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 7.797\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.223\cdot 10^{-4}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 5.730\cdot 10^{-20}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + 5.221\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + 1.628\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}} + 3.093\cdot 10^{-8}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{}} + 1.712\cdot 10^{-2}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.477\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 6.412\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 7.855\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.874\cdot 10^{-8}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 9.758\cdot 10^{-24}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + 2.602\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + 2.477\cdot 10^{-16}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}} + 1.606\cdot 10^{-11}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{2!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.354\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 5.779\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 5.669\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.124\cdot 10^{-8}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 9.431\cdot 10^{-24}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + 2.214\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}} + 8.585\cdot 10^{-17}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}{{{\bar{E}}_{11}}^{}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3} {\delta {\bar{E}}_{11}}^{}}}{\Delta {\bar{\varphi}}_{}}^{3} {\Delta {\bar{E}}_{11}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.065\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.296\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 2.138\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 5.346\cdot 10^{-9}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 3.415\cdot 10^{-24}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}} + 3.273\cdot 10^{-14}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{12}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{12}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{12}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.049\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.265\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 2.168\cdot 10^{-13}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 5.882\cdot 10^{-9}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} - 2.625\cdot 10^{-24}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{4}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.069\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.480\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 5.662\cdot 10^{-14}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}} + 1.961\cdot 10^{-9}{{\gamma}^{{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.197\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.855\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}} + 5.350\cdot 10^{-15}{{\gamma}^{{{{\bar{\varphi}}_{}}^{}}{{{\bar{E}}_{11}}^{}}{{{\bar{E}}_{22}}^{}}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{} {\delta {\bar{E}}_{11}}^{} {\delta {\bar{E}}_{22}}^{}}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 3.155\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}} + 4.790\cdot 10^{-9}{{\gamma}^{{{{\bar{\varphi}}_{}}^{3}}}\frac{1}{{3!}}{\frac{{\delta}^{3}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{3}}}{\Delta {\bar{\varphi}}_{}}^{3}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0}) - 1.537\cdot 10^{-4}{{\gamma}^{{{{\bar{\varphi}}_{}}^{2}}}\frac{1}{{2!}}{\frac{{\delta}^{2}{\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}}{\Delta {\bar{\varphi}}_{}}^{2}}$
${\Psi}_{} = {\Psi}_{}({{{\bar{\varphi}}}}_{0},{{\mathbf{\bar{E}}}}_{0})$


==> figures/model_vol_OLS_Ridge17_nonlocal.tex <==
\begin{align}
\frac{{\delta}^{} {\bar{\varphi}}_{\textrm{OLS-local}}}{{\delta} {{{t}}_{}}^{}} =&~ {\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{E}}_{12}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{11}}^{} {{\bar{E}}_{12}}^{} {{\bar{l}}_{1}}^{}~+~{\gamma}^{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{12}}^{} {{\bar{\varphi}}_{}}^{} {{\bar{l}}_{1}}^{} \label{eq:vol_model_OLS_nonlocal} \\
+&~ {\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{2}}^{}}{{\bar{E}}_{11}}^{} {{\bar{E}}_{22}}^{} {{\bar{l}}_{2}}^{}~+~{\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}}{{\bar{E}}_{11}}^{} {{\bar{E}}_{22}}^{} \nonumber \\ 
+&~  {\gamma}^{{{\bar{E}}_{22}}^{2}}{{\bar{E}}_{22}}^{2}~+~{\gamma}^{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{2}}^{}}{{\bar{E}}_{22}}^{2} {{\bar{l}}_{2}}^{} \nonumber \\ 
+&~  {\gamma}^{{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}{{\bar{\varphi}}_{}}^{} {{\bar{l}}_{1}}^{}~+~{\gamma}^{{{\bar{\varphi}}_{}}^{2}{{\bar{l}}_{1}}^{}}{{\bar{\varphi}}_{}}^{2} {{\bar{l}}_{1}}^{} \nonumber \\ 
+&~  {\gamma}^{{{\bar{E}}_{11}}^{2}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{11}}^{2} {{\bar{l}}_{1}}^{}~+~{\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{11}}^{} {{\bar{l}}_{1}}^{}, \nonumber \\ \nonumber \\
\frac{{\delta}^{} {\bar{\varphi}}_{\textrm{Ridge-local}}}{{\delta} {{{t}}_{}}^{}} =&~ {\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{E}}_{12}}^{}}{{\bar{E}}_{11}}^{} {{\bar{E}}_{12}}^{}~+~{\gamma}^{{{\bar{E}}_{12}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{12}}^{} {{\bar{l}}_{1}}^{} \label{eq:vol_model_Ridge17_nonlocal} \\
+&~ {\gamma}^{{{\bar{E}}_{11}}^{2}}{{\bar{E}}_{11}}^{2}~+~{\gamma}^{{{\bar{E}}_{11}}^{2}{{\bar{l}}_{2}}^{}}{{\bar{E}}_{11}}^{2} {{\bar{l}}_{2}}^{} \nonumber \\ 
+&~  {\gamma}^{{{\bar{E}}_{22}}^{}{{\bar{l}}_{2}}^{}}{{\bar{E}}_{22}}^{} {{\bar{l}}_{2}}^{}~+~{\gamma}^{{{\bar{E}}_{22}}^{2}}{{\bar{E}}_{22}}^{2} \nonumber \\ 
+&~  {\gamma}^{{{\bar{E}}_{11}}^{}}{{\bar{E}}_{11}}^{}~+~{\gamma}^{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{12}}^{} {{\bar{E}}_{22}}^{} {{\bar{l}}_{1}}^{} \nonumber \\ 
+&~ {\gamma}^{{{\bar{\varphi}}_{}}^{2}{{\bar{l}}_{1}}^{}}{{\bar{\varphi}}_{}}^{2} {{\bar{l}}_{1}}^{}~+~ {\gamma}^{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}{{\bar{E}}_{11}}^{} {{\bar{E}}_{22}}^{} {{\bar{l}}_{1}}^{}. \nonumber
\end{align}


==> figures/model_vol_Ridge_17_local.tex <==
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}} + {\gamma}^{{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}}}{{{\bar{E}}_{11}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = {\gamma}^{{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -4.191\cdot 10^{7}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.509\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 3.246\cdot 10^{7}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 3.052\cdot 10^{6}{{{\bar{E}}_{11}}^{}} + 2.726\cdot 10^{5}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 3.606\cdot 10^{8}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 5.877\cdot 10^{6}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + 5.282\cdot 10^{6}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + 3.990\cdot 10^{5}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} - 5.527\cdot 10^{7}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} + 3.800\cdot 10^{5}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -7.318\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 7.204\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 1.798\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 1.664\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 4.276\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 5.386\cdot 10^{5}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 5.203\cdot 10^{3}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + 1.672\cdot 10^{2}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + 9.165\cdot 10^{1}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}} - 8.700\cdot 10^{3}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -7.557\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 7.443\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 1.777\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 1.641\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 4.201\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 5.325\cdot 10^{5}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 5.135\cdot 10^{3}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + 1.740\cdot 10^{2}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} + 4.727{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{2}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -5.379\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 5.326\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 2.065\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 1.957\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 5.401\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 3.675\cdot 10^{5}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 3.552\cdot 10^{3}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}} + 1.104\cdot 10^{2}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -2.305\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 2.359\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 1.767\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 1.668\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 6.079\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 6.859\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 6.802\cdot 10^{2}{{{\bar{E}}_{22}}^{2}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -1.807\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.891\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 1.760\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 1.663\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 5.945\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}} - 3.481\cdot 10^{2}{{{\bar{E}}_{11}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -1.755\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.839\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 2.165\cdot 10^{4}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 2.040\cdot 10^{2}{{{\bar{E}}_{11}}^{}} + 5.518\cdot 10^{1}{{{\bar{E}}_{22}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{N}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -1.303\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.361\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 2.871\cdot 10^{3}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}} + 2.744\cdot 10^{1}{{{\bar{E}}_{11}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -1.815\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.885\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}} - 2.391\cdot 10^{1}{{{\bar{E}}_{11}}^{}{{\bar{\varphi}}_{}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = -1.744\cdot 10^{4}{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}} + 1.820\cdot 10^{2}{{{\bar{E}}_{12}}^{}{{\bar{\varphi}}_{}}^{}{{\bar{l}}_{1}}^{}}$
$\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} = 2.711{{{\bar{E}}_{12}}^{}{{\bar{E}}_{22}}^{}{{\bar{l}}_{1}}^{}}$

